EcoServe: Enabling Cost-effective LLM Serving with Proactive Intra- and Inter-Instance Orchestration

Existing LLM serving strategies can be categorized based on whether prefill and decode phases are disaggregated: non-disaggregated (NoDG) or fully disaggregated (FuDG). However, the NoDG strategy leads to strong prefill-decode interference and the FuDG strategy highly relies on high-performance interconnects, making them less cost-effective. We introduce EcoServe, a system that enables cost-effective LLM serving on clusters with commodity interconnects. EcoServe is built on the partially disaggregated (PaDG) strategy, applying temporal disaggregation and rolling activation for proactive intra- and inter-instance scheduling. It first disaggregates the prefill and decode phases along the time dimension within a single instance to mitigate inter-phase interference and enhance throughput. Next, it coordinates multiple instances and cyclically activates them to ensure the continuous availability of prefill processing, thereby improving latency. Thus, EcoServe's basic serving unit is the macro instance, within which multiple instances collaborate. It further integrates an adaptive scheduling algorithm to route requests in a macro instance and a mitosis scaling approach to enable fine-grained capacity scaling. Beyond delivering high goodput, EcoServe excels in load balancing, hardware cost, parallelism compatibility, and even engineering simplicity compared to existing solutions. When serving 30B- and 70B-scale models on a production-level cluster with 32 NVIDIA L20 GPUs using commodity Ethernet, EcoServe averagely improves goodput by 82.49%, 86.17%, 122.76%, and 126.96% over four representative NoDG and FuDG systems.

==> tex-copy/Background.tex <==
\section{Background and Motivation}

\subsection{LLM Generative Tasks}
\label{sec:llmdecoding}

\begin{figure}[!t]
    \centering    \includegraphics[width=0.75\linewidth]{fig/gen-task.pdf}
    \vspace{-10pt}
    \caption{The generate process of LLM generative task.}
    \label{fig:gen-task}
    \vspace{-10pt}
\end{figure}

Modern LLM generative tasks follow the autoregressive decoding process and predict the next token given an input sequence.
During this process, intermediate states, known as KV cache, are generated at each token position.
Through maintaining KV cache in memory, the modern LLM serving systems can eliminate most redundant computation in this iterative process.
Based on whether the KV cache has been generated, the inference process is divided into prefill and decode phases.
The detailed process of the LLM generative task inference is illustrated in Figure~\ref{fig:gen-task}.
The prefill phase deals with the newly-incoming prompt (in green), often comprising many tokens, and processes these tokens concurrently to generate a new token (in blue).
The prefill phase also initializes the KV cache (in gold).
Next, benefiting from KV cache, each step of the decode phase only processes one new token generated by the previous step.

The running process of LLM generative tasks introduces some key features.
First, the prefill and decode phases have significant computational differences. For the prefill phase, it processes many tokens in parallel and easily becomes the compute-bound workload.
In contrast, the decode phase is more constrained by the memory bandwidth for it has a similar level of I/O compared to the prefill phase and only processes a single token for a single request.
Thus, a very small batch size is sufficient for the prefill phase to saturate computational resources, while the decode phase tends to require a batch size of several hundreds.
Second, LLM generative task inference requires a massive amount of memory.
In addition to weights, hundreds of requests coexist in the decode phase and KV cache contributes significantly to memory usage, especially under the long-context scenarios.
For example, the KV cache of a single token in the Llama-30B~\cite{touvron2023llama} occupies 1.52 MB, and 400 requests with an average length of 300 would require approximately 178 GB of memory.
Since the batch size during the decode phase is crucial for fully utilizing the computing units, memory capacity becomes a key constraint on performance.
Third, LLM generative tasks involve a more complex variable-length problem.
Both input and output lengths are random, and it is difficult to determine the output length until the inference is complete.

\subsection{Cost-effective LLM Serving}

\begin{table}[t]
\caption{Serve a 7B model in 4 NVIDIA RTX 4090 GPUs using data parallelism or model parallelism.}
\vspace{-8pt}
\label{tab:moredbetter}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{cccccc}
\hline
         &  \begin{tabular}[c]{@{}c@{}}\textbf{Device}\\  \textbf{Memory}\end{tabular} &   \begin{tabular}[c]{@{}c@{}}\textbf{Total}\\  \textbf{Weights}\end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{Weights}\\ \textbf{Per GPU}\end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{Token}\\  \textbf{Number}\end{tabular} \\ \hline \hline
Data Para. & 96GB & 56GB          & 14GB            & 34304         \\
Model Para. & 96GB & 14GB          & 3.5GB           & 108800       \\ \hline
\end{tabular}
\vspace{-10pt}
}
\end{table}

% cost effectiveness can be more important
Evaluating the quality of LLM serving can be multifaceted.
Newly introduced metrics include time to first token (TTFT) for the prefill phase and time per output token (TPOT) for each request during the decode phase.
However, due to the resource-intensive nature of LLM inference workloads, many LLM serving systems prioritize cost-effectiveness as a first-class concern.
For example, the popular LLM serving system vLLM~\cite{vllm2024} adopts a throughput-oriented scheduling strategy.
Some systems~\cite{gao2024cost, yu2023stateful,deepseekv2, sheng2023flexgen} have started to adopt a cache layer, such as host memory or even disk, to improve throughput and reduce costs, at the expense of user experience.

% a single device cannot satisfy the resource requirement
As models continuously grow larger and long-context requirements surge, both weights and KV cache consume more memory, making the memory capacity an important performance constraint.
First, the memory capacity should be sufficient for accommodating the model weights.
Commonly used LLM can have 7B, 13B, 30B, 70B, or even more weights, exceeding the memory capacity of most devices, especially these commodity devices such as NVIDIA A10 (24GB), 4090 (24GB), and L20 (48GB).
In addition to weights, the remaining capacity should be able to accommodate a large amount of KV cache to ensure that enough requests can be processed in parallel during the decode phase.
Therefore, sufficient memory capacity is essential for ensuring cost-effective LLM serving.
For example, Table~\ref{tab:moredbetter} shows the memory usage of different strategies when serving a 7B model on 4 NVIDIA RTX 4090 GPUs.
The data parallel approach splits requests across devices, with each device having one copy of the model.
The model parallel approach splits the model and places each fragment on a different device.
As a result, vLLM reports that only 34304 tokens of KV cache can be placed in memory using the data parallel approach, while 108800 tokens of KV cache can be accommodated using the model parallel approach.
With more tokens of KV cache, more requests can be processed in parallel during the decode phase and better saturate devices.

% This approach has two clear benefits:
% 1) Without separation, all nodes are treated equally, making scheduling easier; 2) Inlining chunked prefill into the decoding batch can improve the computational intensity of the decoding batch, leading to better MFU.
% However, after careful consideration, we decided to maintain Mooncake’s disaggregated architecture. A request’s prefill is inlined into the decoding batch only when it can be forwarded without chunking and without compromising the TBT SLO. There are two main reasons for this decision: 1) Prefill nodes require different cross-node parallelism settings to handle long contexts (§4.1). 2).

\subsection{Opportunities of Pipeline Parallelism}

\begin{figure}[t]
    \centering    \includegraphics[width=0.75\linewidth]{fig/multigpu.pdf}
    \vspace{-10pt}
    \caption{The multi-GPU architecture.}
    \label{fig:multigpu}
    \vspace{-10pt}
\end{figure}
 
To increase memory capacity within a single inference instance, two major approaches are commonly used: offloading and parallelization. 
This section analyzes their features when applied to the multi-GPU architecture.
Figure~\ref{fig:multigpu} illustrates the popular multi-GPU architecture widely used in serving LLMs, where multiple GPUs connect to a single CPU.
GPUs are capable of intercommunication via the PCIe switch. 
Furthermore, certain high-performance GPUs enable direct communication through specialized cables, like NVIDIA's NVLINK, which significantly enhances their communication efficiency but also largely raises the node price.

\begin{figure}[!t]
    \centering    \includegraphics[width=0.95\linewidth]{fig/moremem.pdf}
    \vspace{-10pt}
    \caption{Offloading and parallel approaches.}
    \label{fig:moremem}
    \vspace{-10pt}
\end{figure}

As shown in Figure~\ref{fig:moremem}(a), a single inference instance can acquire more memory capacity through offloading data to secondary storage.
While this approach performs well in high-throughput inference when the CPU-to-GPU ratio is 1:1, it encounters severe PCIe contention in a multi-GPU architecture when multiple GPUs simultaneously offload data to host memory.

\begin{figure}[!t]
    \centering    \includegraphics[width=0.95\linewidth]{graph/background_TD_Pipe.pdf}
    \vspace{-10pt}
    \caption{Execution time breakdown of the prefill phase using the tensor parallel approach in a multi-GPU architecture.}
    \label{fig:background_TD}
    \vspace{-10pt}
\end{figure}

Moreover, Figure~\ref{fig:moremem}(b) and (c) show the tensor parallel (TP) and pipeline parallel (PP) approaches.
TP shards each layer across multiple GPUs, with the model weights and KV cache being equally distributed across GPU workers.
It demands frequent communications that a single Transformer layer necessitates two rounds of all-reduce operations.
We deliver distributed inference case studies of Llama-30B~\cite{touvron2023llama} on two nodes without specialized cables in FP16.
To demonstrate strong scalability, we reduce the number of layers in the model to fit into fewer devices and report the running results, shown in Figure~\ref{fig:background_TD}.
Notably, the model is composed of layers with the same structure, so reducing the number of layers does not affect its computational or communication characteristics.
The overall execution time on the L20 node is reduced by 1.84$\times$ when increasing the number of devices from 1 to 4.
Despite the reduction in total execution time, communication time accounts for 47.39\% of the total time on 4 devices.
On the A100 node, the overall execution time is only reduced by 1.64$\times$, with communication time consuming up to 53.9\% of the total time on 4 devices.
Thus, the tensor parallel approach heavily relies on interconnection capability and leaves computational resource idle for long period. 
%如何能看出来资源被浪费了？ 只能说明通信瓶颈大吧？
% or: 
% suffers from significant communication bottleneck.

Compared to TP, PP splits a model layer-wise, where each device is responsible for a subset of layers. 
It only requires a single point-to-point communication with a much smaller data volume every few layers.
The largely-reduced communication makes PP a promising approach to support goodput LLM serving, especially on commodity hardware that high-performance connectivity like NVLINK is unavailable.
Although PP is intensively studied in the deep learning training, 
the imbalanced pipeline workloads and complex data dependencies of LLM inference still prevent it from being the primary choice.
% the complex data dependencies and varying computational characteristics of LLM inference still prevent it from being the primary choice.

\subsection{Batching Strategy for Pipeline Parallelism}
\label{sec:batching}
To fully utilize modern GPUs, the batching technique is commonly adopted for processing deep learning workloads, where multiple samples are processed simultaneously to expose high parallelism and provide considerable hardware performance improvements.
LLM serving systems rely on separate batching and hybrid batching.
% LLM serving systems also rely on the batching technique.
% Separate batching and hybrid batching are used in LLM serving.

Separate batching packs requests exclusively during the prefill phase and solely during the decode phase. Given that these two phases exhibit distinct performance characteristics, i.e. compute-bound and memory-bound, the prefill phase saturates GPU computation even at a batch size of just one, while the decode phase requires a batch size in hundreds.
At each time, the inference instance will stay either in the prefill phase or in the decode phase.
By contrast, hybrid batching combines requests of both prefill and decode phases, and organizes them in hybrid batches.
For a newly-arrived request, it can join an arbitrary batch and start the execution more immediately.

When integrating these two batching approaches into the pipeline parallelism, they present distinct advantages and disadvantages.
For the separate batching, it is intuitive to manage batches with only the prefill phase and we can launch them continuously, for there is no inter-batch data dependency problem.
It is also convenient to manage batches with only the decode phase to achieve the inter-batch load balance, for each decode step of a request fixes to process a single token and has a similar workload.
However, if we mix them up, the data dependency and the load imbalance will result in severe bubble problems.
Moving to the hybrid batching, it is essential to address data dependencies in all batches as decode steps within each batch obey an iterative order.
Despite mitigation approaches like chunked-prefill, the highly random input and output lengths still result in an extremely uneven ratio between prefill and decode phases ~\cite{qin2024mooncake}.
Both batching approaches suffer from bubble problems.
% Achieving inter-batch load balance remains challenging.
% \wyx{This unevenness can still cause bubble problems.}


\subsection{Spatially-Disaggregated Architecture}

Spatially-disaggregated architecture~\cite{qin2024mooncake, zhong2024distserve, patel2023splitwise, hu2024memserve, jin2024pdser} is a popular system design for serving LLMs.
It employs the separate batching, processing the prefill and decode phases in different instances, with the KV cache being transferred between these instances.
With the spatially-disaggregated abstraction, each instance focuses solely on a single phase or even a specific phase type with a particular input feature.
This apparent abstraction makes the serving system more effective in handling different inputs and suited for serving massive amounts of requests.
However, it also requires to balance workloads between different instances.

==> tex-copy/Conclusion.tex <==
\section{Conclusion}

To achieve the high-throughput LLM serving, especially on bandwidth-constrained commodity hardware, we propose the temporally-disaggregated pipeline parallelism architecture.
Around this novel architecture, we identify key concerns and introduce the LLM serving system, TD-Pipe.
Basically, TD-Pipe disaggregates the prefill phase and decode phase in the temporal dimension.
To better exploit the architecture,TD-Pipe decouples the execution plane and the control plane for better device coordination.
In addition, TD-Pipe designs solutions for optimizing the prefill-to-decode and decode-to-prefill switching timing selection, and dynamically balancing the inter-batch workloads during the decode phase.
Experimental results demonstrate that TD-Pipe outperforms existing tensor parallel and pipeline parallel approaches by up to 2.53$\times$ and 2.29$\times$, respectively, when scaling  to 4 GPUs on PCIe nodes.

==> tex-copy/Design.tex <==
\section{The Design of TD-Pipe}

\begin{figure*}[htbp]
    \centering    \includegraphics[width=0.95\linewidth]{fig/overview.pdf}
    \vspace{-10pt}
    \caption{The system overview of TD-Pipe.}
    \label{fig:overview}
    \vspace{-10pt}
\end{figure*}

The key idea of TD-Pipe lies in the temporally-disaggregated pipeline parallelism architecture which disaggregates the prefill and decode phases in the temporal dimension for scheduling in the pipeline parallelism.
Basically, TD-Pipe aims to achieve goodput LLM serving in the multi-GPU architecture, particularly on commodity nodes without additional interconnection cables.

Figure~\ref{fig:overview} demonstrates the overall design of TD-Pipe.
At first, TD-Pipe follows a hierarchical-controller structure, which abstracts the system into a centralized engine and a distributed runtime. 
The centralized engine is responsible for batch scheduling based on memory capacity, request status, and profiling results, and then launching tasks to workers of distributed runtime.
The distributed runtime is responsible for detailed execution and each worker only knows what data and which device it should communicate.
With the hierarchy-controller structure, TD-Pipe enables control of devices and execution in pipeline parallelism.

Next, TD-Pipe identifies the fundamental requirements in the temporally-disaggregated pipeline parallelism architecture and addresses them by three novel approaches.
First, the AI-based greedy prefill approach delays and determines the timing for switching from prefill to decode.
It performs more prefills within a fixed memory capacity by predicting output lengths and simulating the memory usage.
Second, the inter-batch work stealing approach reduces pipeline bubbles caused by random request completion in different batches and it dynamically redistributes workloads from heavy to light batches.
Third, the intensity accumulation approach determines the timing for switching from decode to prefill by comparing the performance cost between the reduced computational intensity and the pipeline bubbles caused by switching.
Finally, TD-Pipe achieves compact pipeline scheduling with only very minimal bubbles in phase switching.

\subsection{Temporally-Disaggregated Pipeline Parallelism}

As stated in Section \S \ref{sec:batching}, each batch of the separate batching can better saturate GPU devices without considering the unbalanced ratio of prefill and decode phases.
However, when migrating the separate batching naively to the pipeline parallelism, it meets serious bubble problems due to data dependencies.
Inspired by the spatially-disaggregated architecture, we tend to disaggregate the prefill phase and the decode phase in the temporal dimension.
The inference instance performs only a single phase type within a relatively long fixed period of time, so as to significantly eliminate pipeline bubbles.
The prefill phase and the decode phase operate in a producer-consumer relationship, where the decode phase relies on the completion of the prefill phase.
Thus, it is still necessary to switch between these two phases.
To enhance this architecture, we aim to reduce phase switching frequency and maintain high efficiency in each phase.

\subsection{Hierarchy-controller System Structure}

To make devices collaborate better, we design the hierarchy-controller system structure for TD-Pipe.
To handle the complex data dependencies and enable asynchronous data transmission simultaneously, as shown in Figure~\ref{fig:overview}, it decouples the scheduling and execution of pipeline tasks, abstracting the centralized engine as the control plane and the distributed runtime as the execution plane.

\subsubsection{Centralized Engine}
The centralized engine manages and controls workers via remote procedure call (RPC).
It is primarily responsible for two distinct stages, i.e. runtime initialization and execution scheduling.
During initialization, it delegates sub-models to workers, initializes the relevant parts of the model and loads parameters into memory.
Execution scheduling deals with batching requests and sending control information to workers.
For the prefill phase, the engine packs prompts and directly sends them to workers until the switching condition is triggered.
For the decode phase, the engine packs decode steps as batches and is also responsible for deleting these completed requests at each iteration.
Additionally, it is worth noting that we treat the CPU as an individual pipeline stage and assign operations such as top-k, top-p, and temperature sampling to the CPU worker to achieve more balanced workloads among workers.

\subsubsection{Distributed Runtime}

Constructing the distributed runtime follows the idea of the SPMD model.
To manage the communication meta-information, such as world size and rank number, a global communication context is initialized.
In this way, after receiving information distributed by the centralized engine, a worker knows what data it should compute, what data it should communicate, and which device it should communicate to based on the global communication context.
We perform the point-to-point communication between pipeline stages asynchronously.

\subsection{AI-based Greedy Prefill Approach}

\begin{algorithm}[!t]
\setlength{\textfloatsep}{0.5cm}
\setlength{\floatsep}{0.5cm}
\setlength{\intextsep}{-5em}
\KwData{\textbf{kvUsage}: Predicted kv cache usage map at future sampling points.  \textbf{kvCapacity}: System kv cache capacity. \textbf{futurePoints}:  Step points for future decision-making}
\SetKwFunction{CheckSwitch}{CheckSwitch}
\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{updateUsage}{UpdateUsage}
\SetKwFunction{schedule}{SchedulePrefill}
\Fn{\CheckSwitch{kvUsage,  kvCapacity}}{
    maxUsage $\gets$ 0 \;
    \ForEach{usage $\in$ kvUsage}{
        \If{usage > maxUsage}{
            maxUsage $\gets$ usage \;
        }
    }
    \If{maxUsage > kvCapacity}{
        Switch to decode\;
    }
    \Else{
        Remain in prefill\;
    }
}
\Fn{\updateUsage{prefillRequest, kvUsage}}{
    inputLen $\gets$ getInputLen(prefillRequest)\;
    predictLen $\gets$ getPredictLen(prefillRequest)\;
    \ForEach{futurePoint $\in$ futurePoints}{
        \If{futurePoint $\leq$ predictLen}{
            kvUsage[futurePoint] += (inputLen + futurePoint)\;
        }
    }
}

\Fn{\schedule{kvUsage,  kvCapacity}}{
    % \tcp{applying continuous batching}
    batch = getPrefillBatch().Launch()\;
    \ForEach{request $\in$ batch}{
        \updateUsage{request, kvUsage}
    }
    \CheckSwitch(kvUsage,  kvCapacity)
}
\caption{Prefill-to-Decode Switch Algorithm}
\label{algo:memusage}
% \vspace{-5pt}
\end{algorithm}

% 在intro或者bg的时候也提一下重计算？作为节约内存的技术
After performing the prefill phase, TD-Pipe requires to determine the timing for switching from prefill to decode.
To reduce the switching frequency between the prefill and decode phase, TD-Pipe tends to execute more prefills before switching to the decode phase.
However, as memory usage continually increases during the decode phase, performing too many prefills consumes most of the memory, leading to frequent re-computation or offloading in the decode phase, which results in a significant performance drop.
Unfortunately, output lengths are unknown until requests complete and the peak memory usage is also unknown.

To determine how many prefills should be launched without largely exceeding the memory capacity during the decode phase, we propose the AI-based greedy prefill approach.
If we could know input and output lengths of all requests, we could calculate the total memory usage and determine the switching timing.
Furthermore, during the decode phase where all requests progress together, some requests generate new KV cache while others complete, freeing the associated KV cache.
By simulating the memory usage throughout the entire process, we can perform prefills more aggressively.

The AI-based greedy prefill approach introduces an additional network to predict output lengths.
Through adding additional prompts or training an additional independent small transformer model, existing works~\cite{zheng2024response, hu2024inference} successfully predict output lengths.
However, the prompt-adding approach alters the original behavior, and the small model approach struggles to remain consistent with the original large model.
For scheduling tasks that require to predict output lengths before prefills, the small model approach is widely adopted.
In contrast, our AI-based greedy prefill introduces an additional head (a single linear layer) on top of the last hidden states of the LLM to predict the output length range of requests.
The head-adding approach is adopted based on four facts:
1) Knowing the output length until the prefill is complete satisfies the requirement for our memory usage prediction task.
2) Predicting with the LLM's hidden states leverages more information and can produce more credible results.
3) Since our goal is to predict the total memory usage range, errors in prediction can be mitigated by accumulating the output length range across hundreds of requests.
4) \textbf{Although existing models support extremely long-context inference, the output length is usually within a reasonable length.} (In the multi-turn conversation dataset shareGPT V3~\cite{hfshareGPT}, 99.14\% of output sentences are shorter than 1024 tokens, and 99.96\% shorter than 2048 tokens).

% It is noted that a small batch size that right saturates the device will be chosen in the prefill phase.
% This is because the prediction results will only be known until the last device in the pipeline finishes execution, and a large batch size could enlarge the delay. \wyx{what delay?}
%最后这句话也没能读明白

To simulate the memory usage for the subsequent decoding steps after performing new prefills, as in Algorithm~\ref{algo:memusage}, we design a dynamic programming (DP) algorithm to simulate this process after each prefill completes without introducing significant overhead.
To simplify the computational complexity, we designate certain decode steps in the future for decision-making, referred to as \textit{futurePoints}.
For example, we only check whether the memory usage in the 32nd, 64th, 96th, ..., 992nd, 1024th decode steps exceeds the memory capacity.
After newly launching a batch, the algorithm updates the KV cache usage at these decode steps (\textit{futurePoints}) by checking whether the predicted output lengths exceeds certain decode steps.
With the future KV cache usage, we can determine the timing for switching from prefill to decode by checking whether there exists a \textit{futurePoint} that the memory usage is larger than the memory capacity.

\subsection{Inter-batch Work Stealing Approach}

\begin{figure}[!t]
    \centering    \includegraphics[width=0.95\linewidth]{fig/app-2.pdf}
    \vspace{-10pt}
    \caption{The inter-batch work stealing approach. \textbf{bs(wi)} represents the batch size with stealing and \textbf{bs(wo)} represents the batch size without stealing. Here we assume the execution time is strictly proportional to the batch size and some requests normally finish in this process.}
    \label{fig:app-2}
    % \vspace{-10pt}
\end{figure}

Because of data dependencies, the inter-batch load imbalance can result in pipeline bubbles.
To maintain load balance, the batch scheduler of the centralized engine must ensure that workloads remain evenly distributed across batches throughout the entire decode phase.

First, TD-Pipe requires to identify scheduling target for ensuring load balance.
The execution time of a single decode step is determined by two factors: batch size and the lengths of KV cache.
The batch size used in the decode phase can reach several hundreds and the range of KV cache lengths varies even more, making it impossible to accurately estimate the execution time.
Since linear operations (only relate to batch size) in Transformer models generally dominate execution time across most sequence lengths and large batch sizes can mitigate execution time fluctuations arising from different KV cache lengths, we consider batch size as the sole metric for indicating load balance between batches.

Second, at the beginning, TD-Pipe divides the requests into batches equal to the number of GPUs, with each batch containing the same number of requests.
As the decode phase progresses, requests in different batches complete randomly and the workloads of different batches constantly change, resulting in imbalanced workloads.
In addition, the batch scheduler can only know the batch size of a single batch at any given moment, while the batch sizes of other batches remain unknown.
Therefore, TD-Pipe requires a dynamic scheduling strategy based on only the local information.

At last, the inter-batch work stealing approach employs the idea of sliding window to balance inter-batch workloads on-the-fly.
Figure~\ref{fig:app-2} demonstrates a slightly extreme example of how this approach gradually achieves load balance and performance benefits.
When each batch completes a decode step, this approach calculates the average of its current batch size and the historical batch sizes of other batches.
Then, the current batch size is compared with the average batch size, and a decision is made to either add or remove requests from this batch.
If requests are removed, they will be temporarily set aside, waiting to be added to subsequent batches.
If requests are added, it will check whether there are requests from previous batches that have been set aside.
Balanced inter-batch workloads can be achieved through this iterative process.
In the lower part of Figure~\ref{fig:app-2}, the imbalanced workloads quickly trend towards balance, and the reduced pipeline bubble translates into performance gains.


\subsection{Intensity Accumulation Approach}

\begin{figure}[!t]
    \centering    \includegraphics[width=0.95\linewidth]{fig/app-3.pdf}
    \vspace{-10pt}
    \caption{The intensity accumulation approach.}
    % alpha point文中也没出现
    \label{fig:app-3}
    \vspace{-10pt}
\end{figure}

In the temporally-disaggregated pipeline architecture, the decode phase acts as the consumer. 
As the decode phase progresses, some requests complete, causing the batch size to decrease and leading to a drop in computational intensity. 
If the computational intensity continues to drop, the decode phase would operate in low efficiency. 
However, if we switch to the prefill phase as soon as decode efficiency drops, frequent switching could create bubbles and harm performance.
To handle this dilemma, the intensity accumulation approach aims to determine the optimal timing for switching from decode to prefill.

As shown in Figure~\ref{fig:app-3}, the intensity accumulation approach compares the performance drop caused by decreases in computational intensity with the pipeline bubbles resulting from phase switching. 
If the performance drop exceeds the impact of the pipeline bubbles, the system should switch from decode to prefill. 
While this comparison is conceptually straightforward, quantifying the performance drop and the pipeline bubbles is not as intuitive.
For the performance drop, we measure it by accumulating the decreases in computational intensity.
In detail, we profile the execution time and calculate the average execution time per request using a sufficiently large batch size.
We refer to the average execution time per request under high computational intensity as the \textit{baseline time}.
As the decode phase progresses, the average time per request increases as computational intensity decreases.
When the average time exceeds a certain threshold (to mitigate misjudgments caused by performance fluctuation), we begin accumulating the performance drop. 
For each step, we record the wasted execution time due to decreased computational intensity by:
\begin{equation}
    Total \, Execution \, Time - (Batch \, Size \times Baseline \, Time)
\end{equation}

Next, we estimate the wasted execution time due to pipeline bubbles by combining real-time data with hyperparameter information.
As shown in Figure~\ref{fig:app-3}, there are two parts of pipeline bubbles marked in red lines.
For the left part, since the execution time of the current decode step and the upcoming prefill can be known, we can accurately calculate the wasted time due to pipeline bubbles in this part.
For the right part, the bubbles are determined by the longest prefill and the first decode step following the prefill phase.
Thus, we use the hyperparameter information, that the batch size of the prefill phase is determined by setting a total prompt length, to estimate the execution time of bubbles.
Combining these two parts, the intensity accumulation approach can estimate the wasted execution time due to pipeline bubbles.
% 没懂这里historical information指什么
% 另外图中还有一种bubble是prefill和prefill之间的不用管么 (这个是prefill造成的bubble)



==> tex-copy/Discussion.tex <==
\section{Future Work and Discussion}
\label{sec:discussion}

It is promising to further improve this temporally-disaggregated pipeline parallelism architecture by the following aspects:
\begin{itemize} [leftmargin=*]
    \item TD-Pipe is primarily designed for high-throughput and cost-effective LLM serving, with less emphasis on latency-related metrics. However, if there is a backlog of requests, TD-Pipe can outperform other approaches in latency metrics. Furthermore, by implementing upper-level scheduling and allocating requests to TD-Pipe instances operating in the appropriate phase, this architecture shows promise in achieving low latency at high throughput.
    \item The output length prediction is a use case of AI for AI systems and is worth further study. Potential methods include fine-tuning predictions with parameter-efficient methods, dataset design, and increasing prediction frequency.
    \item Tensor parallelism and pipeline parallelism have distinct advantages. Pipeline parallelism has low communication demands but requires more memory to gain high computational intensity, while tensor parallelism is the opposite.    
\end{itemize}


==> tex-copy/Evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We implement TD-Pipe on top of vLLM~\cite{vllm2024}.
We evaluate the effectiveness of TD-Pipe by comparing it with SOTA approaches and report the KV cache memory usage fluctuation during running.
Additionally, we conduct an ablation study to assess the impact of our proposed approaches.

\subsection{Experimental Setup}

\begin{table}[!t]
% \vspace{-10pt}
\caption{GPU Configurations}
\vspace{-10pt}
\label{tab:gpus}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c c c c c}
\hline
\textbf{  Device  }&  \textbf{   FP16 Tensor Core   } & \textbf{   Bandwidth   } & \textbf{   Memory   } & \textbf{   AllReduce   }\\ 
\hline \hline
L20 &  119.5 TFLOPS & 864 GB/s   &   48  GB      &   17.85 GB/s\\
A100 &  312 TFLOPS & 1,935 GB/s  &   80  GB      &   14.82 GB/s\\
\hline
\end{tabular}
}
\vspace{-10pt}
\end{table}

\noindent\textbf{Node testbed.} 
We deploy TD-Pipe on two multi-GPU nodes as shown in Table~\ref{tab:gpus}.
One has 4 NVIDIA L20 GPUs (48GB) and another one has 4 NVIDIA A100 GPUs (80GB).
These two nodes all communicate through PCIe switch with a peak all-reduce bandwidth at 17.85 GB/s and 14.82 GB/s respectively.
Specifically, we use Pytorch$\sim$v2.3.1, vLLM$\sim$v0.5.3, CUDA$\sim$12,4, and NCCL$\sim$2.20.5.

\begin{table}[!t]
% \vspace{-10pt}
\caption{Model Specifications.}
\vspace{-10pt}
\label{tab:models}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{ccccccc}
\hline
\textbf{Name}                        & \textbf{Parameters} & \textbf{Layers} & \textbf{Heads} & \textbf{Hidden Size} &\textbf{ Prec.} \\ \hline\hline
\multicolumn{1}{c}{Llama2-13B} & 26GB & 40     & 40    & 5,120  & FP16       \\
\multicolumn{1}{c}{Llama2-34B} & 68GB & 64     & 48    & 8,192  & FP16     \\
Llama2-70B                    & 140GB & 80     & 64    & 8,192  & FP16  \\ \hline
\end{tabular}
}
\vspace{-10pt}
\end{table}
\noindent\textbf{Model setup.}
We choose Llama2~\cite{touvron2023llama2} in different model sizes.
As detailed in Table~\ref{tab:models}, they are Llama2-13B, Llama2-34B, and Llama2-70B.
Notably, the 34B and 70B models use the group query attention (GQA) technique, which results in a smaller KV cache capacity for the same token count.
% GQA不引用一下么 @doujiangsu

\noindent\textbf{Baseline Methods.}
We compare TD-Pipe with some recently released approaches implemented in vLLM~\cite{vllm2024}:
\begin{itemize}[leftmargin=*]
    \item \textbf{TP+SB}: The tensor parallel approach is integrated with separate batching. This method requires two All-reduce synchronizations in each transformer layer, and serves as the default approach in vLLM.
    \item \textbf{PP+SB}: The pipeline parallel approach is integrated with separate batching. This method requires limited communications but suffers from a severe bubble problem.
    \item \textbf{PP+HB}: The pipeline parallel approach is integrated with hybrid batching, along with the chunked-prefill approach. This method requires limited communications but still experiences the bubble problem.
\end{itemize}
Also, we employ the re-computation strategy where the KV cache of recently arrived requests will be freed once memory capacity is saturated, to deal with memory overflow issues.
Once model weights is loaded, the system profiles the remaining memory capacity and calculates how many KV cache blocks can be accommodated.

\noindent \textbf{Dataset and Metrics.}
The popular multi-turn conversation dataset, shareGPT V3~\cite{hfshareGPT}, is adopted in the evaluation.
The dataset contains around 53,000 samples, with each sample includes indefinite number of conversation rounds.
Following the benchmarking method used in vLLM, we filter input sentences with a length of less than 1024 tokens.
These input sentences are fed into the target models to generate new output sentences, constructing 86,612 input and output pairs.
For output length prediction training in the AI-based greedy prefill approach, 9,300 samples are used as the training dataset, 500 samples as the validation dataset, and all the other samples are used as the test dataset.
These datasets are uniformly sampled from the original dataset.
For performance evaluation, we randomly sample 5,000 input sentences as requests and use throughput (tokens/s) as the metric for TD-Pipe is a throughput-oriented LLM serving system. 
Each run of serving 5,000 requests consumes around half an hour.
% If time permit, add TTFT to evaluation

\subsection{Overall Performance Evaluation}
\begin{figure*}[htbp]
    \centering    \includegraphics[width=0.9\linewidth]{graph/overall_perf.pdf}
    \vspace{-10pt}
    \caption{Overall performance.}
    \label{fig:overall-perf}
    \vspace{-10pt}
\end{figure*}

We compare TD-Pipe against baseline methods and present their overall throughput results for processing 5,000 input sequences.
Taking the ratio between memory capacity and model size into consideration, we select four node-model combinations: L20 + Llama2-13B, L20 + Llama2-34B, A100 + Llama2-34B, and A100 + Llama2-70B, and scale them from 1 to 4 GPUs.
We train prediction heads for these models respectively and report details in Section~\ref{sec:appeva1}.

Figure~\ref{fig:overall-perf} presents the throughput results, with the red box indicating the linear speed up.
In almost all cases, TD-Pipe presents advantages over other approaches, especially when the device number is 4.
For 4-device cases in all node-model configurations, TD-Pipe achieves up to 2.53$\times$ more throughput over TP+SB; 2.65$\times$ more throughput over PP+SB; and 2.29$\times$ more throughput over PP+HB.
Comparing PP+SB and PP+HB, it shows that the combination of hybrid batching and chunked-prefill approach can indeed optimize the pipeline parallelism by improving the inter-batch load balance.
% \wyx{Comparing PP+SB and PP+HB \wyx{, it} shows that the chunked-prefill approach can indeed optimize hybrid batching efficiency by improving inter-batch load balance.}
% PP+SB 和 PP+HB 有两个不同： 1、batching方式 2、是否使用chunked-prefill approach
% 为什么能直接下结论说这里的收益是来自于chunked-prefill approach
% 此外，你2.4的最后一段还说了SB能够更好地achieve inter-batch balance，这不是矛盾了么

TD-Pipe demonstrates super-linear speedup as the number of GPUs increases from 1 to 4, largely outperforming other pipeline parallel approaches.
For example, when the GPU number scales from 2 to 4, the throughput of L20 + Llama2-34B grows 3.24$\times$.
When scaling from 2 to 4 GPUs, both the computing capability and the memory capacity are doubled.
On the one hand, the increased computing capability contributes to the speedup.
On the other hand, the increased memory capacity can be used for accommodating more KV cache and the computational intensity during the decode phase is largely improved.
Under the dual effects, TD-Pipe's throughput achieves super-linear improvement.
In comparison, the other two pipeline parallel approaches, PP+SB and PP+HB, show less improvement. This is because they are less impacted by memory capacity, and longer pipeline stages on more devices exacerbate their bubble problems.

Although TD-Pipe outperforms TP+SB in all our evaluation cases, it is clear that they each have distinct use scenarios.
Comparing L20 + Llama2-34B and A100 + Llama2-34B, we can first observe that A100 + Llama2-34B has significantly higher throughput than that of L20 + Llama2-34B, which aligns with the hardware specifications.
Additionally, we can also notice that the throughput ratio between TD-Pipe and TP+SB varies between the two setups.
When performing with 4 GPUs, TD-Pipe achieves a performance improvement of 1.46$\times$ faster compared to TP+SB on the L20 node, while TD-Pipe is 1.74$\times$ faster than TP+SB on the A100 node.
This is related to many aspects, including the memory bandwidth, computing capability, memory capacity, and interconnection ability.
On the one hand, as shown in Table~\ref{tab:gpus}, the A100 is much faster than L20 in terms of both memory bandwidth and computing capability, while the interconnection ability is lower.
Thus, TP+SB on the A100 node is more constrained by the interconnection, where TD-Pipe is much less reliant.
On the other hand, since all requests can be batched together 
using TP and requests are divided into multiple batches using PP, TP tends to achieve higher computational intensity than PP, while PP is more constrained by the memory capacity.
As a result, PP benefits more from the fact the A100 node's greater memory capacity.
Notably, since we record the overall throughput from the start of the first prefill to the finish of all decode batches, the execution tail of PP approach is less efficient compared to TP approach for its batch size is smaller. Nevertheless, our PP approach is still more effective than TP approach.


\subsection{KV Cache Memory Usage}
\begin{figure}[htbp]
    \centering    \includegraphics[width=0.9\linewidth]{graph/memory_usage.pdf}
    \vspace{-10pt}
    \caption{The KV cache memory usage fluctuation.}
    \label{fig:memory_usage}
    \vspace{-10pt}
\end{figure}

Figure~\ref{fig:memory_usage} illustrates the ratio between the practical KV cache memory usage and the total memory allocated for KV cache as inference progresses. 
Initially, the KV cache memory usage increases continuously until the GPU memory is fully utilized. 
This process includes both the prefill and decode phases and can trigger re-computation as the memory uses up. 
After a short period where the memory is fully occupied, the memory usage begins to decline.
The memory usage experiences multiple ups and downs, occasionally decreasing before reaching full capacity. 
Ultimately, the memory usage continuously decreases as the decode phase continues until all requests are completed.
% In fact, this execution tail causes our throughput measurement of PP approaches to be lower, as they operate with smaller batch sizes compared to TP approach at the tail.
% \wyx{Nevertheless, our PP approach is still more effective than TP approach.(?)}
% Ultimately, the decode phase continues until all requests are completed, \wyx{and the memory usage continuously decreases to 0}.
% Notably, since we record the execution time from start to finish and calculate the throughput, the execution tail of PP approach is less efficient compared to TP approach for its batch size is smaller.

\subsection{Ablation Study}
This section illustrates how each approach impacts TD-Pipe.
% We classify them into two categories.
% The AI-based greedy prefill and intensity accumulation approaches are both designed to determine better switching timing, replacing the approach of manually setting hyperparameters.
% The inter-batch work stealing approach optimizes inter-batch load balance, and while beneficial, it can be removed.
% while beneficial, it can be removed
%是什么意思？虽然有益但是可以被移除？

\subsubsection{Approach-1: AI-based Greedy Prefill}
\label{sec:appeva1}

\begin{figure}[htbp]
    \centering    \includegraphics[width=0.9\linewidth]{graph/prefill-to-decode.pdf}
    \vspace{-10pt}
    \caption{Ablation study for prefill-to-decode switching.}
    \label{fig:prefill-to-decode}
    \vspace{-12pt}
\end{figure}
To demonstrate how effective the AI-based greedy prefill can determine the timing for switching from prefill to decode, we design a hyperparameter called the KV cache occupancy ratio to replace the AI-based greedy prefill approach.
For example, when we set this ratio as 50\%, the prefill will switch to decode once 50\% KV cache blocks are occupied.
Figure~\ref{fig:prefill-to-decode} shows the throughput results, demonstrating that our approach outperforms all other manually selected switching points.
For the hyperparameter approach, it requires human experience and numerous experiments.
This result illustrates that our AI-based greedy prefill approach can determine a fairly good switching point, and it can dynamically fit the constantly changing requests.

In detail, for output length prediction, we train prediction heads that support 16-class classification for all three models respectively.
In other words, we only predict the output length range of a request.
By analyzing the prediction accuracy, we observe that the output length prediction is not so accurate.
For example, in the 16-class output length prediction, adding a head to Llama2-13B only achieves 40\%, 62\%, and 76\% accuracy for 0 adjacent intervals, 1 adjacent interval, and 2 adjacent intervals, respectively.
In this prediction head, the input is the hidden state of the first token, and the output is the probability of classification results. This simple mapping relationship makes it highly prone to overfitting during training. Rather than accurately learning to predict output length, we are more inclined to believe that the model has learned the heavy-tailed distribution of the entire dataset.

\subsubsection{Approach-2: Inter-batch Work Stealing}

\begin{figure}[h]
    \centering    \includegraphics[width=0.9\linewidth]{graph/approach2.pdf}
    \vspace{-10pt}
    \caption{Ablation study for the decode batch load balance.}
    \label{fig:approach2}
    \vspace{-10pt}
\end{figure}

We report throughput results with (\textbf{wi}) or without (\textbf{wo}) the inter-batch work stealing approach in Figure~\ref{fig:approach2}.
The load balance scheduling at the timing for switching from prefill to decode is still kept and only the dynamic balance during the decode phase is removed.
L20 + 34B and A100 + 70B have 1.14$\times$ and 1.07$\times$ throughput improvement after activating our inter-batch work stealing approach, validating its effectiveness.

\subsubsection{Approach-3: Intensity Accumulation}

\begin{figure}[h]
    \centering    \includegraphics[width=0.9\linewidth]{graph/decode-to-prefill.pdf}
    \vspace{-10pt}
    \caption{Ablation study for decode-to-prefill switching.}
    \label{fig:decode-to-prefill}
    \vspace{-12pt}
\end{figure}

Like evaluating the AI based greedy prefill approach, we introduce a hyperparameter called the request finish ratio to replace the intensity accumulation approach.
For example, if this ratio is set to 50\%, the decode phase will switch to prefill once 50\% of the requests have completed.
In Figure~\ref{fig:decode-to-prefill}, the manually selected points perform well even when the ratio is somewhat extreme, due to the large memory capacity in these cases.
In comparison, the intensity accumulation approach achieves the highest throughput, illustrating its effectiveness.

==> tex-copy/Introduction.tex <==
\section{Introduction}
\label{sec:intro}
% background: LLM increase
% generative tasks 
Large language models (LLMs) \cite{brown2020language, touvron2023llama, zeng2022glm, zhang2022opt, touvron2023llama2} demonstrate significant capabilities and have facilitated the development of a wide range of intelligent applications, including code assistants~\cite{AmazonCode, GithubCopilot}, conversational engines~\cite{cai, chatgpt}, and search engines~\cite{bingsearch, googlebard}.
Since the widespread adoption of LLMs, serving them cost-effectively becomes unprecedentedly important.
In other words, maximizing the throughput under given hardware has become the top priority in most cases \cite{vllm2024, sheng2023flexgen}.
However, achieving this is not trivial.

% large memory requirement and 4090 -> multi-GPU architecture -> weak interconnection and low memory
A prominent feature of LLM generative inference is its substantial memory requirement.
On the one hand, LLMs are renowned for their massive weights.
The number of parameters can be 7B, 13B, 30B, 70B, 175B, and so on, taking up tens or even hundreds of gigabytes of memory.
On the other hand, LLM generative tasks require storing a large capacity of KV cache, which can exceed the memory consumed by the weights.
The LLM generative inference generates tokens iteratively, and this process is divided into two phases, prefill and decode.
The prefill phase processes the input prompt and stores the generated keys and values of all tokens (KV cache) to avoid repeated computation.
With the KV cache, the decode phase iteratively processes each token generated from the previous iteration and continuously appends the key and value of the new token to the KV cache, until the serving of the given prompt is completed.
To saturate the capability of computing devices, a large number of requests should be batched and processed together during the decode phase \cite{yu2022orca, agrawal2024taming, zhong2024distserve, lee2024infinigen}, requiring substantial memory capacity to store the KV cache.
To meet the requirement in terms of large memory, existing systems typically employ offloading and parallel approaches.


% offloading what problems?
Offloading approaches run an LLM with limited GPU memory by offloading data to the secondary storage and retrieving it when the data is accessed. 
By carefully optimizing the computation schedule and tensor placement, existing offloading approaches~\cite{sheng2023flexgen, 2022deepspeed} can perfectly hide the communication between GPU memory and the secondary storage among computation, achieving considerable throughput with only a single GPU.
Unfortunately, offloading approaches inherently suffer from severe contention problems.
Specifically, under the commonly-used multi-GPU architecture, several GPUs share the only one channel linked with CPU, and consequently there is serious bandwidth contention on CPU’s root complexes when multiple GPUs offload data simultaneously.
% First, despite the significant differences in resource usage types, communication and computation kernels still share some resources, leading to contention problems during concurrent execution.




% parallel what problems
Parallel approaches distribute a single LLM inference instance across multiple devices.
Tensor parallelism~\cite{shoeybi2019megatron, dudu2024liger} is widely used in existing LLM serving systems~\cite{nvidia2023fast, aminabadi2022deepspeed, vllm2024, tensorrt2024} due to its simplicity.
Through splitting each layer into symmetric fragments and distributing fragments to devices, devices performs the similar computation, and they communicate with collective primitives, following the single program multiple data (SPMD) model.
However, due to the frequent and intensive synchronizations, considerable communication overhead makes it inefficient.
% Communication can occupy half of the time when using commodity hardware with weak interconnections and up to 20\% of the time even when using advanced hardware with NVLINK.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/pipeline_bubble.pdf}
    \vspace{-10pt}
    \caption{Bubbles in LLM pipeline parallel inference.}
    \label{fig:pipeline_bubble}
    \vspace{-10pt}
\end{figure}

In comparison, pipeline parallelism~\cite{huang2019gpipe, dudu2024liger} splits a model by layers and only transfers activations between cut-off layers.
This low-communication feature makes it a promising approach for fully exploiting the computational capabilities of devices.
However, due to the imbalanced pipeline workloads and complex data dependencies, achieving compact scheduling is challenging, and bubbles always exist.
Figure~\ref{fig:pipeline_bubble} presents the running process of batching prefill and decode phases separately and scheduling them in an interleaved manner, as in most practical LLM serving systems~\cite{vllm2024, tensorrt2024,qin2024mooncake}.
The imbalanced workloads come from two aspects.
First, different batch sizes lead to different decode step workloads, resulting in the inter-batch imbalance.
Second, the prefill-decode imbalance exists as the execution of prefill usually takes much longer time than a decode step. 
Likewise, the data dependencies also come from two aspects.
On the one hand, inter-layer data dependency requires data to be processed in the current layer before entering to the next layer for processing.
One the other hand, inter-decode-step data dependency exists as the execution of generating the next token cannot start until the previous iteration completes.
Therefore, bubble problems always hinder the practical use of pipeline parallelism in serving LLMs. 

% First, the inter-batch imbalance results in bubbles.
% This occurs because the execution of generating the next token cannot start until the previous iteration completes.
% If the workloads between batches are imbalanced, bubbles appear.
% Second, the imbalance between prefill and decode phases also results in bubbles.
% Although there is no strict dependency between these phases, the longer execution time of prefill phase still leads to bubbles.
% Consequently, frequent switching between prefill and decode phases has severe bubble problem.
% \wyx{
% In Figure~\ref{fig:pipeline_bubble}, the imbalanced pipeline workloads and complex data dependencies cause massive pipeline bubbles.
% The imbalanced workloads come from two aspects.
% First, different batch sizes lead to different decode step workloads, resulting in the inter-batch imbalance.
% Second, the prefill-decode imbalance exists as the execution of prefill usually takes much longer than a decode step. 
% Likewise, the data dependencies also come from two aspects.
% On the one hand, inter-layer data dependency exists due to the serialization feature of LLMs, which requires data to be processed in the current layer before entering to the next layer for processing.
% One the other hand, inter-deocde-step data dependency exists as the execution of generating the next token cannot start until the previous iteration completes.
% Therefore, it necessitates the careful scheduling of prefill and decode of different batches in the pipeline parallelism. 
% }

An alternative approach to mitigate the pipeline bubble problem is the combination of the chunked-prefill approach~\cite{agrawal2024taming} and the hybrid batching~\cite{yu2022orca}.
Initially, hybrid batching is proposed to optimize the time to first token (TTFT) metric by unifying prefill and decode in a single hybrid batch.
When applying to pipeline parallelism, the chunked-prefill approach splits the prefill computation into chunks and mixes these prefill chunks with decode, aiming to achieve better inter-batch load balance.
However, this approach relies on the prefill-to-decode ratio and struggles with requests of constantly changing lengths, with significant bubbles still unsolved.
% vLLM~\cite{vllm2024} achieves around a 10\% improvement in pipeline parallelism using the chunked-prefill approach, with significant bubbles still remain.

In order to better exploit the pipeline parallelism for goodput LLM serving, we propose TD-Pipe, an LLM serving system based on the temporally-disaggregated pipeline parallelism architecture.
The key idea is to disaggregate the prefill and decode phases in the temporal dimension, or rather, to reduce the prefill-decode switching frequency as much as possible.
TD-Pipe is inspired by the popular spatially-disaggregated architecture~\cite{qin2024mooncake, zhong2024distserve, patel2023splitwise, hu2024memserve,jin2024pdser}, which places the prefill and decode phases on different instances and transfer KV cache between them.
It should be noted that the spatially-disaggregated architecture is suitable for customizing services in giant companies, since it requires a powerful interconnected system and a comprehensive software design.

TD-Pipe identifies key issues in supporting the temporally-disaggregated pipeline parallelism architecture and provides solutions.
It includes a hierarchy-controller system structure and three novel approaches.
The hierarchy-controller structure addresses the problem of inefficient collaboration between devices in a pipeline.
Since different devices perform consecutive layers of a model and LLM inference workloads are generally irregular in terms of input and output lengths, the device-to-device transfer has to be in a blocking style.
The hierarchy-controller decouples the scheduling from execution by introducing the distributed runtime (execution plane) and the centralized engine (control plane), enabling unblocked transmission.

Next, to enhance efficiency throughout the entire execution process, three approaches are proposed.
First, to delay the timing of switching from prefill to decode, we propose the AI-based greedy prefill approach.
To reduce the switching frequency, it is reasonable to complete prefill phase for more requests without exceeding the memory capacity.
We add an additional head at the end of a LLM to predict the output length and perform prefills aggresively, considering that some requests finish and the related KV cache will be freed.
Second, to reduce pipeline bubbles in the decode phase, we propose the inter-batch work stealing approach.
% \wyx{the inter-decode-step data dependency
Since requests will finish randomly and result in imbalance, this approach dynamically balances the number of requests between batches.
Third, to determine the optimal timing of switching from decode to prefill, we propose the intensity accumulation approach.
As the decode phase progresses, requests continuously end, and the reduced computational intensity of batches leads to efficiency degradation.
Once the computational intensity starts to reduce, we accumulate the performance loss and compare it with the decode-to-prefill switching overhead to determine the switching timing.
In summary, we make the following contributions:
\begin{itemize}[leftmargin=*]
    \item We identify causes of bubble problem in serving LLM generative tasks using the pipeline parallelism. % (\S \ref{sec:intro})   
    \item We design the novel temporally-disaggregated pipeline parallelism architecture targeting at goodput LLM serving, which disaggregates the prefill and decode phases in the temporal dimension.
    \item We identify potential issues of exploiting the temporally-disaggregated pipeline parallelism architecture and present TD-Pipe with solutions.
    \item We evaluate TD-Pipe and show its efficiency. % (\S \ref{sec:evaluation})
    \item We discuss further chances for TD-Pipe.  % (\S \ref{sec:discussion})
\end{itemize}

 
% It includes the hierarchy-controller system structure for better coordinating devices in pipeline parallelism. It includes the the AI-based greedy prefill approach, the inter-batch work stealing approach, and the intensity accumulation approach to help determine the prefill-decode switching timing and reduce the inter-batch load imbalance.

==> tex-copy/RelatedWork.tex <==
% \section{Related Work}

==> tex/Motivation.tex <==
\section{Motivation}

\begin{table*}[!t]
\begin{tabular}{ccccccc}
\hline
  & SLOs  & Throughput & Data Movement Overhead &  Engineering Complexity & Infrastructure Cost & Parallelism Compatibility \\ \hline \hline
NoDG + separate batching   &  &  &  & \\ 
NoDG + hybrid batching   &  &  &  & \\ 
FuDG + intra-node &  &  &  &  \\ 
FuDG + inter-node &  &  &  &  \\ 
PaDG &  &  &  &  \\ \hline
\end{tabular}
\end{table*}

\subsection{SLOs versus Throughput}

\subsection{Cost-effective LLM Serving}
% capatibility with parallel strategies
% NoDG

\subsection{Inter-instance Collaboration}


Furthermore, the high computational and memory demands of LLMs necessitate the adoption of parallel strategies in inference infrastructure, wherein multiple GPUs are utilized in a single instance, exposing the limitations of NoDG and FuDG strategies.
LLM inference generally adopts tensor parallelism and pipeline parallelism.
Tensor parallelism partitions each operation across multiple devices, adhering to the single program multiple data (SPMD) model, while pipeline parallelism partitions the target model by layers, processing multiple stages in a pipelined manner.
Tensor parallelism involves extensive collective communication, which significantly hinders the achievement of high throughput.
Pipeline parallelism relies much less on interconnections; however, addressing inter-stage load imbalance is challenging and critical for minimizing pipeline bubbles.
Thus, the NoDG strategy is incompatible with pipeline parallelism, as maintaining consistent workloads across different batches is challenging due to the significant disparity between prefills and decodes.
Moving to the FuDG strategy, the massive transfer of KV cache can interfere with collective communication in tensor parallelism, competing for valuable network bandwidth.


% \subsection{Cost-effective LLM Serving}
% % capatibility with parallel strategies

% NoDG

% % \subsection{Request Scheduling Overhead}
% % 大量节点调度延迟高，CPU受不了，而少量节点不会影响。

% % \subsection{Request Rate Fluctuation}
% % 请求速率：在长期波动，在短期稳定。
